Preserving Causal Constraints in Counterfactual Explanations for Machine Learning Classifiers

To construct interpretable explanations that are consistent with the original ML model, counterfactual examples---showing how the model's output changes with small perturbations to the input---have been proposed. This paper extends the work in counterfactual explanations by addressing the challenge of feasibility of such examples. For explanations of ML models in critical domains such as healthcare and finance, counterfactual examples are useful for an end-user only to the extent that perturbation of feature inputs is feasible in the real world. We formulate the problem of feasibility as preserving causal relationships among input features and present a method that uses (partial) structural causal models to generate actionable counterfactuals. When feasibility constraints cannot be easily expressed, we consider an alternative mechanism where people can label generated CF examples on feasibility: whether it is feasible to intervene and realize the candidate CF example from the original input. To learn from this labelled feasibility data, we propose a modified variational auto encoder loss for generating CF examples that optimizes for feasibility as people interact with its output. Our experiments on Bayesian networks and the widely used ''Adult-Income'' dataset show that our proposed methods can generate counterfactual explanations that better satisfy feasibility constraints than existing methods.. Code repository can be accessed here: \textit{https://github.com/divyat09/cf-feasibility}

==> learning_constraints.tex <==
\section{Learning Causal Constraints}
While the proposed methods assumed that constraints were known, an important challenge is to learn causal constraints from data. Here we extend the OracleGenCF method to learn constraints from the labels provided by a feasibility Oracle. We assume that the domain-expert provides a set of variables that may have constraints and provides the type of constraint (e.g., monotonicity). For simplicity, let us assume only pairwise constraints and assume that the constraint type is \textit{monotonicity}. Below is our approach.

Loop through for each pair of features ($x_1, x_2)$:
\begin{itemize}
    \item \textbf{Detect constraint.} Consider the distribution $\Pr_F(X_1, X_2)$ and $\Pr_I(X_1, X_2)$ in the labelled feasible and infeasible CFs respectively. Conduct a statistical test to check if they are significantly different, and thus a constraint exists.
    \item \textbf{Identify the causal direction.} If there is a constraint, consider the conditional distributions $\Pr_F(X_2|X_1)$ and $\Pr_F(X_1|X_2)$. A simple test is: if $X_2$ changes without any change in $X_1$, then $X_1$ causes $X_2$ (and vice-versa).
\end{itemize}

Evaluation and more details are in the Suppl. Materials. Extending the approach to beyond pairwise and simple constraints (e.g., independence constraints) is future work. 
